Unified-IO: A Unified Model for Vision, Language, and Multi-Modal Tasks

We propose Unified-IO, a model that performs a large variety of AI tasks spanning classical computer vision tasks, including pose estimation, object detection, depth estimation and image generation, vision-and-language tasks such as region captioning and referring expression, to natural language processing tasks such as question answering and paraphrasing. Developing a single unified model for such a large variety of tasks poses unique challenges due to the heterogeneous inputs and outputs pertaining to each task, including RGB images, per-pixel maps, binary masks, bounding boxes, and language. We achieve this unification by homogenizing every supported input and output into a sequence of discrete vocabulary tokens. This common representation across all tasks allows us to train a single transformer-based architecture, jointly on over 90 diverse datasets in the vision and language fields. Unified-IO is the first model capable of performing all 7 tasks on the GRIT benchmark and produces strong results across 16 diverse benchmarks like NYUv2-Depth, ImageNet, VQA2.0, OK-VQA, Swig, VizWizGround, BoolQ, and SciTail, with no task-specific fine-tuning. Code and demos for Unified-IO are available at: https://unified-io.allenai.org.

==> table/tasks_v1.tex <==
\begin{table}[t]
\renewcommand{\dashlinedash}{2pt}
\renewcommand{\dashlinegap}{2pt}
\newcommand{\band}{\rowcolor{gray!10}}
\newcommand{\checkcol}{p1.5cm}
\newcolumntype{M}{>{\centering\arraybackslash}p{0.9cm}}
\renewcommand{\indent}{\hspace{0.2cm}}
\setlength\tabcolsep{3pt}
\renewcommand{\arraystretch}{1.25}
\center
  \resizebox{\textwidth}{!}{
  \begin{tabular}{l  c c c c :  M M M M  :  M M M M}
  \toprule
   & \multicolumn{4}{c}{Data} & \multicolumn{4}{c}{Input Modalities} & \multicolumn{4}{c}{Output Modalities} \\ 
    \cmidrule(r){2-5}
    \cmidrule(r){6-9}
    \cmidrule(r){10-13}
   & Datasets & Size & Percent & \multicolumn{1}{c}{Rate}  & Text & Image & Sparse & \multicolumn{1}{c}{Dense} & Text & Image & Sparse & \multicolumn{1}{c}{Dense} \\
  \midrule

\band \textbf{Image Synthesis}  & 14 & 56 & 43.0 & 18.7 &  & \checkmark & \checkmark & \checkmark & \checkmark & - & \checkmark & - & \checkmark \\
\indent Image Synthesis from Text & 9 & 55 & 41.9 & 16.7 & COCO & \checkmark & - & - & - & - & \checkmark & - & - \\
\indent Image Inpainting & 3 & 1.2 & 0.9 & 1.5 & VG & \checkmark & \checkmark & \checkmark & - & - & \checkmark & - & - \\
\indent Image Synthesis from Seg. & 2 & 0.22 & 0.2 & 0.6 & LVIS & \checkmark & - & - & \checkmark & - & \checkmark & - & \checkmark \\
\band \textbf{Text Grounding}  & 10 & 8.2 & 6.3 & 12.5 &  & \checkmark & \checkmark & \checkmark & - & - & - & \checkmark & - \\
\indent Object Localization & 3 & 6 & 4.6 & 7.1 & Open Images & \checkmark & \checkmark & - & - & - & - & \checkmark & - \\
\indent Object Detection & 3 & 1.9 & 1.5 & 3.6 & Open Images & - & \checkmark & - & - & - & - & \checkmark & - \\
\indent Keypoint Estimation & 1 & 0.14 & 0.1 & 0.7 & COCO & - & \checkmark & \checkmark & - & - & - & \checkmark & - \\
\indent Referring Expression & 3 & 0.13 & 0.1 & 1.1 & RefCoco & \checkmark & \checkmark & - & - & - & - & \checkmark & - \\
\band \textbf{Dense Labelling}  & 6 & 2.4 & 1.8 & 6.2 &  & \checkmark & \checkmark & - & - & - & - & - & \checkmark \\
\indent Surface Normal Estimation & 2 & 0.21 & 0.2 & 1.1 & Framenet & - & \checkmark & - & - & - & - & - & \checkmark \\
\indent Depth Estimation & 1 & 0.048 & 0.1 & 0.4 & NYU Depth & - & \checkmark & - & - & - & - & - & \checkmark \\
\indent Object Segmentation & 3 & 2.1 & 1.6 & 4.7 & LVIS & \checkmark & \checkmark & - & - & - & - & - & \checkmark \\
\band \textbf{Image Captioning}  & 7 & 31 & 23.7 & 12.5 &  & - & \checkmark & \checkmark & - & \checkmark & - & - & - \\
\indent Webly Supervised Captioning & 3 & 26 & 19.7 & 8.8 & CC12M & - & \checkmark & - & - & \checkmark & - & - & - \\
\indent Human Supervised Captioning & 3 & 1.4 & 1.1 & 1.7 & VizWiz & - & \checkmark & - & - & \checkmark & - & - & - \\
\indent Region Captioning & 1 & 3.8 & 2.9 & 2.0 & VG & - & \checkmark & \checkmark & - & \checkmark & - & - & - \\
\band \textbf{Image Classification}  & 9 & 22 & 16.8 & 12.5 &  & \checkmark & \checkmark & \checkmark & - & \checkmark & - & - & - \\
\indent Object Categorization & 3 & 6 & 4.6 & 4.4 & Open Images & - & \checkmark & \checkmark & - & \checkmark & - & - & - \\
\indent Image Classification & 6 & 16 & 12.2 & 8.1 & Imagenet & \checkmark & \checkmark & - & - & \checkmark & - & - & - \\
\band \textbf{Vision \& Language}  & 16 & 4 & 3.0 & 12.5 &  & \checkmark & \checkmark & \checkmark & - & \checkmark & - & - & \checkmark \\
\indent VQA & 13 & 3.3 & 2.5 & 10.4 & VQA 2.0 & \checkmark & \checkmark & - & - & \checkmark & - & - & - \\
\indent Relationship Detection & 2 & 0.64 & 0.5 & 1.9 & VG & - & \checkmark & \checkmark & - & \checkmark & - & - & - \\
\indent Grounded VQA & 1 & 0.0065 & 0.1 & 0.1 & VizWiz & \checkmark & \checkmark & - & - & \checkmark & - & - & \checkmark \\
\band \textbf{NLP}  & 33 & 7.1 & 5.4 & 25.0 &  & \checkmark & - & - & - & \checkmark & - & - & - \\
\indent Masked Language Modelling & 2 & 0 & 0.1 & 12.5 & Wikipedia & - & - & - & - & - & - & - & - \\
\indent Question Answering & 13 & 1.7 & 1.3 & 5.2 & SQuAD & \checkmark & - & - & - & \checkmark & - & - & - \\
\indent Text Summarization & 1 & 3.8 & 2.9 & 2.5 & Gigaword & \checkmark & - & - & - & \checkmark & - & - & - \\
\indent Text Classification & 17 & 1.6 & 1.2 & 4.8 & MNLI & \checkmark & - & - & - & \checkmark & - & - & - \\
\band \textbf{Unsupervised NLP}  & 0 & 0 & 0.1 & 0.0 &  & - & - & - & - & - & - & - & - \\
\textbf{All Tasks} & 95 & 130 & 100.0 & 100.0 & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\

  \bottomrule
\end{tabular}}

\caption{\small{.}}
\label{tab:tasks}
\vspace{-10pt}
\end{table}

